Detection of Small Scale Components in Power Law Spectra

Spectra in astroparticle physics are commonly approximated by simple power laws. The steeply falling nature of these power laws, however, makes the detection of additional components rather challenging. This holds true especially, if the additional components are small compared to the established ones. Energy spectra of muon neutrinos are an interesting example of such a scenario, where the conventional and astrophysical components to the spectra have been established by the use of different analysis methods, such as likelihood fits or spectral deconvolution. The prompt component, although expected from theoretical models, has not yet been experimentally observed. Furthermore, the extraction of physics parameters is challenged by the large systematic uncertainties, especially at high energies. This contribution presents a different approach to the analysis of power-law spectra, which is based on functional data analysis. The method itself and its implications are discussed using muon and neutrino energy spectra as an example.

==> Makefile <==
TeXOptions = \
  -lualatex \
  --output-directory=build \
  --interaction=nonstopmode \
  --halt-on-error

all: build/main.pdf 

build/main.pdf: FORCE | build
#	latexmk $(TeXOptions)  Optik.tex
	pdflatex $(TeXOptions) main.tex
	bibtex build/main.aux
	pdflatex $(TeXOptions) main.tex
	pdflatex $(TeXOptions) main.tex
	
FORCE:

build:
	mkdir -p build

clean:
	rm -rf build


.PHONY: all clean FORCE

